MolKD: Distilling Cross-Modal Knowledge in Chemical Reactions for Molecular Property Prediction

How to effectively represent molecules is a long-standing challenge for molecular property prediction and drug discovery. This paper studies this problem and proposes to incorporate chemical domain knowledge, specifically related to chemical reactions, for learning effective molecular representations. However, the inherent cross-modality property between chemical reactions and molecules presents a significant challenge to address. To this end, we introduce a novel method, namely MolKD, which Distills cross-modal Knowledge in chemical reactions to assist Molecular property prediction. Specifically, the reaction-to-molecule distillation model within MolKD transfers cross-modal knowledge from a pre-trained teacher network learning with one modality (i.e., reactions) into a student network learning with another modality (i.e., molecules). Moreover, MolKD learns effective molecular representations by incorporating reaction yields to measure transformation efficiency of the reactant-product pair when pre-training on reactions. Extensive experiments demonstrate that MolKD significantly outperforms various competitive baseline models, e.g., 2.1% absolute AUC-ROC gain on Tox21. Further investigations demonstrate that pre-trained molecular representations in MolKD can distinguish chemically reasonable molecular similarities, which enables molecular property prediction with high robustness and interpretability.

==> section/7-Others.tex <==
\paragraph{Reproducibility statement.}
The source code along with a README file with instructions on how to run these experiments is attached in the supplementary material. In addition, more discussions about dataset descriptions and statistics, hyper-parameters for our proposed model, and experimental settings are detailed in Appendix~\ref{sec:appendix-A}.

\paragraph{Ethics statement.}
In this work, our studies are not related to human subjects, practices to data set releases, potentially harmful insights, discrimination/bias/fairness concerns, and also do not have legal compliance or research integrity issues.
All datasets we used are curated from public data sources,
and are released under a license that allowed for public access. The datasets are all anonymized.
We develop a novel and practical method to incorporate chemical domain knowledge for popular molecular property prediction problems. Therefore, we do not foresee any particular concerns related to its ethical aspects or future societal consequences.
However, advanced computational chemistry tools may pose the risk of misuse, \eg, for the development of chemical weapons. Our studies, to the best of our knowledge, do not promote misuse any more than computational chemistry research.

==> table/classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}
\centering
\small
\caption{Results of molecular property prediction on classification tasks~(metric: AUC-ROC). The first block is the conventional methods without pre-training thus we omit their \emph{\#Pre-training data}. We split the pre-training methods in the second to the fourth block according to three method categories introduced in Sec.~\ref{sec:related}. The results in the first four blocks are taken from their original papers and ``-'' means they do not report the corresponding results. ``Z'', ``C'', ``P'', ``Gu'', ``Ge'', `U-4'', and ``U-1'' in the \emph{\#Pre-training data} column denote the used pre-training data, which are the abbreviation of ZINC15~\citep{sterling2015zinc}, ChEMBL~\citep{gaulton2012chembl}, PubChem~\citep{kim2019pubchem}, GuacaMol~\citep{brown2019guacamol}, GEOM~\citep{axelrod2022geom}, USPTO-479k~\citep{wang2021chemical}, and USPTO-500-MT~(140k)~\citep{lu2022unified} respectively.}
%ZINC15~\citep{sterling2015zinc}, ChEMBL~\citep{gaulton2012chembl}, PubChem~\citep{kim2019pubchem}, GuacaMol~\citep{brown2019guacamol}, GEOM~\citep{axelrod2022geom}, USPTO-479k~\citep{wang2021chemical}, and USPTO-500-MT~(140k)~\citep{lu2022unified}
% ZINC15, ChEMBL, PubChem, GuacaMol, GEOM, USPTO-479k, and USPTO-500-MT~(140k)
\vspace{-0.5em}
\label{table:classification}
\setlength{\tabcolsep}{4pt}
\scalebox{0.73}{
\begin{tabular}{c|cccccc|cc}
\toprule\toprule
                 & BACE        & BBBP     & ClinTox     & HIV        & SIDER      & Tox21     & \#Params (M)               & \begin{tabular}{c}\#Pre-training\\data (M)\end{tabular}    \\ \midrule
AttentiveFP      & $0.784$        & $0.643$        & $0.847$        & $0.771$        & $0.606$        & $0.761$        & -                           &                              \\
GCN              & $0.716$        & $0.718$         & $0.625$        & $0.740$        & $0.536$        & $0.709$        & $1.04$                        &                              \\
D-MPNN           & -            & $0.708$        & $0.906$        & $0.752$        & $0.632$        & $0.688$        & $1.41$                        &                              \\
SchNet           & $0.766_{\pm0.011}$ & $0.848_{\pm0.022}$ & $0.715_{\pm0.037}$ & $0.702_{\pm0.034}$ & $0.539_{\pm0.037}$ & $0.727_{\pm0.023}$ & 2.20                        & \multirow{-4}{*}{*}          \\ \midrule
Mol2vec          & $0.862_{\pm0.027}$ & $0.872_{\pm0.021}$ & $0.841_{\pm0.062}$ & $0.769_{\pm0.021}$ & -            & $0.803_{\pm0.041}$ & 4.87                        & $19.90$ (Z+C)         \\
ChemBERTa        & -            & $0.643$        & $0.733$        & $0.622$        & -            & $0.728$        & $56.44$                       & $77.00$ (P)               \\
MolBert          & $0.866$        & $0.762$        & -            & $0.783$        & -            & $0.806$        & $64.42$                       & $1.60$ (Gu)               \\
PretrainGNN & $0.845_{\pm0.007}$ & $0.687_{\pm0.013}$ & $0.726_{\pm0.015}$ & $0.799_{\pm0.007}$ & $0.627_{\pm0.008}$ & $0.781_{\pm0.006}$ & 4.36                        & 2.00 (Z)                 \\
GROVER-base       & $0.878_{\pm0.016}$ & \underline{$0.936_{\pm0.008}$} & $0.925_{\pm0.013}$ & -            & $0.656_{\pm0.006}$ & $0.819_{\pm0.020}$ & $48.39$                       & $11.00$ (Z+C)         \\
MolCLR-GCN       & $0.788_{\pm0.005}$ & $0.738_{\pm0.002}$ & $0.867_{\pm0.010}$ & $0.778_{\pm0.005}$ & $0.669_{\pm0.012}$ & $0.747_{\pm0.008}$ & $1.04$                        & $10.00$ (P)               \\
MolCLR-GIN       & \bm{$0.890_{\pm0.003}$} & $0.736_{\pm0.005}$ & \underline{$0.932_{\pm0.017}$} & $0.806_{\pm0.011}$ & \underline{$0.680_{\pm0.011}$} & $0.798_{\pm0.007}$ & $2.40$                        & $10.00$ (P)               \\ \midrule
GEM              & $0.856_{\pm0.011}$ & $0.724_{\pm0.004}$ & $0.901_{\pm0.013}$ & $0.806_{\pm0.009}$ & $0.672_{\pm0.004}$ & $0.781_{\pm0.001}$ & $1.66$                        & $20.00$ (Z)                \\
GraphMVP         & $0.768_{\pm0.011}$ & $0.685_{\pm0.002}$ & $0.790_{\pm0.025}$ & $0.748_{\pm0.014}$ & $0.623_{\pm0.016}$ & $0.745_{\pm0.004}$ & $3.22$                        & $0.05$ (GE)   \\ \midrule
KCL              & $0.860$         & $0.927$        & $0.898$        & -            & $0.659$        & \underline{$0.825$}        & $1.16$                        & $0.25$ (Z) \\
MolR-GCN         & \underline{$0.882_{\pm0.019}$} & $0.890_{\pm0.032}$ & $0.916_{\pm0.0394}$ & $0.802_{\pm0.024}$ & -            & $0.818_{\pm0.023}$ & $1.98$                        & $0.48$ (U-4)  \\
MolR-TAG         & $0.875_{\pm0.023}$ & $0.895_{\pm0.031}$ & $0.913_{\pm0.043}$ & $0.801_{\pm0.023}$ & -            & $0.820_{\pm0.028}$ & $3.26$                        & $0.48$ (U-4)  \\ \midrule
MolKD$^{-}$      & $0.876_{\pm0.031}$ & $0.902_{\pm0.028}$ & $0.917_{\pm0.039}$ & \underline{$0.811_{\pm0.021}$} & $0.660_{\pm0.048}$ & $0.818_{\pm0.059}$ & $3.26$                        & $0.14$ (U-1)  \\
MolKD (ours)            & $0.872_{\pm0.022}$ & \bm{$0.942_{\pm0.021}$} & \bm{$0.933_{\pm0.041}$} & \bm{$0.816_{\pm0.011}$} & \bm{$0.706_{\pm0.020}$} & \bm{$0.841_{\pm0.032}$} & $0.84$ & $0.14$ (U-1)  \\ \bottomrule\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table*}

==> table/regression.tex <==
\begin{table}{}
\centering
% \small
\caption{Results of molecular property prediction on regression tasks~(metric: RMSE for ESOL and FreeSolv; MAE for QM8).}
\label{table:regression}
\setlength{\tabcolsep}{6pt}
\scalebox{0.8}{
\begin{tabular}{cccc}
\toprule
                 & ESOL       & FreeSolv   & QM8            \\ \midrule
AttentiveFP      & $0.88_{\pm0.03}$ & $2.07_{\pm0.18}$ & $0.0179_{\pm0.0001}$ \\
GCN              & $1.43_{\pm0.05}$ & $2.87_{\pm0.14}$ & $0.0366_{\pm0.0011}$ \\
D-MPNN           & $0.98_{\pm0.26}$ & $2.18_{\pm0.91}$ & \underline{$0.0143_{\pm0.0022}$} \\
SchNet           & $1.05_{\pm0.06}$ & $3.22_{\pm0.76}$ & $0.0204_{\pm0.0021}$ \\ \midrule
PretrainGNN & $1.10_{\pm0.01}$ & $2.76_{\pm0.02}$ & $0.0200_{\pm0.0001}$ \\
GROVER-base       & $0.98_{\pm0.09}$ & $2.18_{\pm0.05}$ & $0.0218_{\pm0.0004}$ \\
MolCLR-GCN       & $1.16_{\pm0.00}$ & $2.39_{\pm0.14}$ & $0.0181_{\pm0.0002}$ \\
MolCLR-GIN       & $1.11_{\pm0.01}$ & $2.20_{\pm0.20}$ & $0.0174_{\pm0.0013}$ \\ \midrule
GEM              & \underline{$0.80_{\pm0.03}$} & $1.88_{\pm0.09}$ & $0.0171_{\pm0.0001}$ \\
GraphMVP         & $1.09$       & -          & -              \\ \midrule
MolKD$^{-}$      & $0.93_{\pm0.06}$ & \underline{$1.64_{\pm0.12}$} & $0.0206_{\pm0.0028}$ \\
MolKD (ours)           & \bm{$0.75_{\pm0.03}$} & \bm{$1.56_{\pm0.16}$} & \bm{$0.0133_{\pm0.0008}$} \\ \bottomrule
\end{tabular}
}
\end{table}
